Learning Equilibria of Simulation-Based Games

We tackle a fundamental problem in empirical game-theoretic analysis (EGTA), that of learning equilibria of simulation-based games. Such games cannot be described in analytical form; instead, a black-box simulator can be queried to obtain noisy samples of utilities. Our approach to EGTA is in the spirit of probably approximately correct learning. We design algorithms that learn so-called empirical games, which uniformly approximate the utilities of simulation-based games with finite-sample guarantees. These algorithms can be instantiated with various concentration inequalities. Building on earlier work, we first apply Hoeffding's bound, but as the size of the game grows, this bound eventually becomes statistically intractable; hence, we also use the Rademacher complexity. Our main results state: with high probability, all equilibria of the simulation-based game are approximate equilibria in the empirical game (perfect recall); and conversely, all approximate equilibria in the empirical game are approximate equilibria in the simulation-based game (approximately perfect precision). We evaluate our algorithms on several synthetic games, showing that they make frugal use of data, produce accurate estimates more often than the theory predicts, and are robust to different forms of noise.

==> approximation.tex <==
Next, we show that several important game-theoretic properties are Lipschitz continuous in utilities.
By applying Lemma~\ref{lem:lipschitz-properties}, we then derive two-sided 
approximation bounds
for these properties.

\begin{definition}[Utilitarian Welfare]
Given a normal-form game $\GameTuple$ with utility function $\Utility$, together with a strategy profile $\StratProfile$, the \mydef{utilitarian welfare} of $\StratProfile$ is defined as
$\Welfare (\Utility, \StratProfile) \doteq \sum_{\PlayerIndex \in \SetOfPlayers} \Utility_\PlayerIndex (\StratProfile)$.
\end{definition}

\begin{definition}[Pessimal and Maximin Values and Maximin Strategies]
Given a normal-form game $\GameTuple$ with utility function $\Utility$, agent $\PlayerIndex$'s \mydef{pessimal value} of the (mixed or pure) strategy $\Strategy$ is defined as $\PessimalValue(\Utility, \PlayerIndex, \Strategy) \doteq \inf_{\StratProfile | \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile).$ 
Agent $\PlayerIndex$'s \mydef{maximin value} is given by
$\MinimaxValue(\Utility, \PlayerIndex) \doteq \sup_{\Strategy \in \StrategySet_\PlayerIndex} \PessimalValue(\Utility, \PlayerIndex, \Strategy)$.
A strategy $\Strategy$ is $\alpha$-\mydef{maximin optimal} for agent $\PlayerIndex$ if $ \PessimalValue(\Utility, \PlayerIndex, \Strategy) \geq \MinimaxValue(\Utility, \PlayerIndex) - \alpha$.
\end{definition}


\begin{definition}[Regret]
Given a normal-form game $\GameTuple$ with utility function $\Utility$, agent $\PlayerIndex$'s \mydef{regret} for playing strategy $\Strategy \in \StrategySet_\PlayerIndex$ rather than strategy $\tilde{\Strategy} \in \StrategySet_\PlayerIndex$ when all other agents are playing strategy profile $\StratProfile$ is defined as
$\MV_{\PlayerIndex} (\Utility, \tilde{\Strategy}, \StratProfile)
    \doteq 
\Utility_\PlayerIndex(\tilde{\StratProfile}) - \Utility_\PlayerIndex(\StratProfile)$, 
where $\tilde{\StratProfile}_j = \StratProfile_j$ for all agents $j \neq \PlayerIndex$ and $\tilde{\StratProfile}_\PlayerIndex = \tilde{\Strategy}$.
\end{definition}


\begin{theorem}[Approximable Properties of Normal-Form Games]
\label{thm:lipschitz-properties}
Given normal-form games $\GameTuple, \GameTuple'$, with utility functions $\Utility$ and $\Utility'$, respectively, such that $\norm{\GameTuple - \GameTuple'}_\infty \leq \epsilon$, the following hold:

\begin{enumerate}

\item \label{thm:lipschitz-properties:welfare} \mydef{Utilitarian Welfare Approximation}:
\vspace{-0.35cm}
\[
\sup_{\StratProfile \in \StratProfileSpace} 
    \left| \Welfare(\Utility, \StratProfile) - \Welfare(\Utility', \StratProfile) \right| 
        \leq 
    \NumberOfPlayers \epsilon
\qquad \text{ and } \qquad
\left| 
    \sup_{\StratProfile \in \StratProfileSpace} \Welfare(\Utility, \StratProfile) 
    - 
    \sup_{\StratProfile' \in \StratProfileSpace} \Welfare (\Utility', \StratProfile') 
\right| 
        \leq 
    \NumberOfPlayers \epsilon
\]
\vspace{-0.3cm}

\item \label{thm:lipschitz-properties:minimax} \mydef{Maximin Optimality}: If strategy $\Strategy$ is $\alpha$-maximin optimal for agent $\PlayerIndex$ in $\GameTuple'$, so that $\PessimalValue(\Utility', \PlayerIndex, \Strategy) 
    \geq 
 \MinimaxValue(\Utility', \PlayerIndex) - \alpha$, then 
$\PessimalValue(\Utility, \PlayerIndex, \Strategy) 
    \geq 
\MinimaxValue(\Utility, \PlayerIndex) - \epsilon - \alpha$.


\item \label{thm:lipschitz-properties:equilibria} \mydef{Approximate Equilibria}: $\Nash(\GameTuple) 
    \subseteq 
\Nash_{2\epsilon}(\GameTuple') 
    \subseteq 
\Nash_{4\epsilon}(\GameTuple),$ and
$\Nash^\diamond(\GameTuple) 
    \subseteq 
\Nash^\diamond_{2\epsilon}(\GameTuple') 
    \subseteq 
\Nash^\diamond_{4\epsilon}(\GameTuple).$

\end{enumerate}
\end{theorem}

\begin{proof}
We show each result through Lemma~\ref{lem:lipschitz-properties} by constructing an appropriate function family and showing it to be Lipschitz w.r.t.{} $\norm{\cdot}_\infty$.

We first show \ref{thm:lipschitz-properties:welfare}.  Take $\F \doteq \{ f(\Utility) \doteq \Welfare(\Utility, \StratProfile) \mid \StratProfile \in \StratProfileSpace \}$.
Now note that utilitarian welfare is $\NumberOfPlayers$-Lipschitz w.r.t.{} $\norm{\cdot}_\infty$, as a uniform $\epsilon$ change to utilities produces a change in utilitarian welfare of no more than $\NumberOfPlayers\epsilon$.
The result then follows via Lemma~\ref{lem:lipschitz-properties}
(\ref{lem:lipschitz-properties:uniform}) and (\ref{lem:lipschitz-properties:opt-val}).

\if 0
\begin{align*}
\sup_{f \in \F} \abs{f(\GameTuple) - f(\GameTuple')} &= \sup_{\StratProfile \in \StratProfileSpace} \abs{\Welfare (\GameTuple, \StratProfile) - \Welfare (\GameTuple', \StratProfile) } & \textsc{Definition of $\F$} \\
 &= \sup_{\StratProfile \in \StratProfileSpace} \smallabs{\sum_{\PlayerIndex \in \SetOfPlayers} \Utility(\StratProfile) - \Utility'(\StratProfile)} & \textsc{Definition of Welfare} \\
 &\leq \sum_{\PlayerIndex \in \SetOfPlayers} \sup_{\StratProfile \in \StratProfileSpace} \abs{\Utility(\StratProfile) - \Utility'(\StratProfile)} & \textsc{Jensen's Inequality} \\
 &\leq N\norm{\GameTuple - \GameTuple'}_\infty = N\epsilon & \textsc{Assumption} \\
\end{align*}
\fi


We now show \ref{thm:lipschitz-properties:minimax}.  Take $\F \doteq \{ f(\Utility) \doteq \PessimalValue(\Utility, \PlayerIndex, \Strategy) \mid \PlayerIndex \in \SetOfPlayers, \Strategy \in \StrategySet_\PlayerIndex \}$.  First note that, for all $\PlayerIndex, \Strategy$, it holds that $\PessimalValue(\Utility, \PlayerIndex, \Strategy)$ is $1$-Lipschitz w.r.t.{} $\norm{\cdot}_\infty$.  To see this, note that a uniform $\epsilon$ change to $\Utility$ either \emph{decreases} $\inf_{\StratProfile | \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex(\StratProfile)$ by up to $\epsilon$, by \emph{decreasing} some $\Utility_\PlayerIndex(\StratProfile)$ with $\StratProfile_\PlayerIndex = \Strategy$ and $\Utility_\PlayerIndex(\StratProfile) \leq \inf_{\StratProfile' | \StratProfile'_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) + \epsilon$, or \emph{increases} $\inf_{\StratProfile | \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile)$ by up to $\epsilon$, by \emph{increasing} some $\Utility_\PlayerIndex (\StratProfile)$ with $\StratProfile_\PlayerIndex = \Strategy$ and $\Utility_\PlayerIndex (\StratProfile) \leq \inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) + \epsilon$.
The result now follows via the definition of $\alpha$-maximin optimality and Lemma~\ref{lem:lipschitz-properties} (\ref{lem:lipschitz-properties:opt-fun}).


\if 0
\begin{align*}
\sup_{f \in \F} \abs{f (\Utility) - f (\Utility')} &= \sup_{\PlayerIndex, \Strategy} \abs{\inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile'_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile')} & \textsc{Definition of $\PessimalValue$} \\
 &= \sup_{\PlayerIndex, \Strategy}\sup_{\StratProfile | \StratProfile_\PlayerIndex = \Strategy}\inf_{\StratProfile' | \StratProfile'_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \Utility'_\PlayerIndex (\StratProfile') & \textsc{Symmetry} \\
\end{align*}

\[
\abs{ \inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile')} = \sup_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy}\inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) -  \Utility'_\PlayerIndex (\StratProfile') \leq  
\]
(to see this, note that decreasing any $\Utility_p(\StratProfile)$ by $\epsilon$ changes the pessimal utility by from $-\epsilon$ to $0$, increases by $0$ to $\epsilon$).  The result now follows via the definition of $\alpha$-maximin optimality and \Cref{lem:lipschitz-properties}.\ref{lem:lipschitz-properties:opt-fun}.
\fi

\if 0
\[
\inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile') - \epsilon \leq \inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile') \leq \inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile') + \epsilon \enspace.
\]

\iftrue
_\infty$ ).
\fi

We first show that $\F$ is a $1$-Lipschitz function family.
\begin{align*}
\sup_{f \in \F} \abs{f (\Utility) - f (\Utility')} &= \sup_{\PlayerIndex, \StratProfile} \abs{\inf_{\StratProfile \mid \StratProfile_\PlayerIndex = \Strategy} \Utility_\PlayerIndex (\StratProfile) - \inf_{\StratProfile' \mid \StratProfile_\PlayerIndex = \Strategy} \Utility'_\PlayerIndex (\StratProfile')} & \textsc{Definition of $\PessimalValue$} \\
\end{align*}


\fi

We now show \ref{thm:lipschitz-properties:equilibria}.  Let $\F \doteq \{ f(\bm{u}) \doteq %
\MV_{\PlayerIndex} (\Utility,  \tilde{\Strategy}, \StratProfile)
\mid 
\PlayerIndex \in \SetOfPlayers, 
\tilde{\Strategy} \in \StrategySet_\PlayerIndex, 
\StratProfile \in \StratProfileSpace \}$.
We first show that $\F$ is a $2$-Lipschitz function family.
\begin{align*}
\sup_{f \in \F} \left| f (\Utility) - f (\Utility') \right| &= \sup_{\PlayerIndex, \StratProfile, \tilde{\StratProfile}} \left| (\Utility_\PlayerIndex (\tilde{\StratProfile})- \Utility_\PlayerIndex (\StratProfile)) - (\Utility_\PlayerIndex' (\tilde{\StratProfile}) - \Utility_\PlayerIndex' (\StratProfile)) \right| & \textsc{Definition of $\MV$} \\[-0.2cm]
&\leq \sup_{\PlayerIndex, \tilde{\StratProfile}} \left| \Utility_\PlayerIndex (\tilde{\StratProfile}) - \Utility_\PlayerIndex' (\tilde{\StratProfile}) \right| + \sup_{\PlayerIndex, \StratProfile} \left| \Utility_\PlayerIndex (\StratProfile) - \Utility_\PlayerIndex' (\StratProfile) \right|  & \textsc{Triangle inequality} \\[-0.05cm]
 &= 2\norm{\GameTuple - \GameTuple'}_\infty & \textsc{Definition of $\norm{\cdot}_\infty$} %
\end{align*}

We use this preliminary result to show equilibrium containment. 
As any pure equilibrium is also a mixed equilibrium, we need only show this containment for mixed equilibria. 
Note that a strategy profile is a Nash equilibrium if the regret of all players for all their strategies is non-negative. 
\begin{align*}
\Nash^\diamond_{\alpha}(\GameTuple) &= \{ \StratProfile \mid \smallsup{\PlayerIndex \in \SetOfPlayers, \tilde{\Strategy} \in \StrategySet^\diamond_\PlayerIndex} \MV_{\PlayerIndex} (\Utility, \tilde{\Strategy}, \StratProfile) + \alpha \geq 0 \} & \textsc{Definition of $\alpha$-Nash Equilibrium} \\[-0.15cm]
& \subseteq \{ \StratProfile \mid \smallsup{\PlayerIndex \in \SetOfPlayers, \tilde{\Strategy} \in \StrategySet^\diamond_\PlayerIndex} \MV_{\PlayerIndex} (\Utility, \tilde{\Strategy}, \StratProfile) + 2 \epsilon + \alpha \geq 0  \} & \textsc{\Cref{lem:lipschitz-properties} (\ref{lem:lipschitz-properties:opt-fun})} \\[-0.15cm]
&= \Nash^\diamond_{\alpha + 2\epsilon}(\GameTuple') & \textsc{Definition of $\GameTuple$}
\end{align*}

\noindent Taking $\alpha = 0$ shows the first case, and taking $\alpha = 2\epsilon$ and flipping $\GameTuple,\GameTuple'$ shows the second.
\end{proof}


We thus see that several useful game-theoretic properties can be approximated with bounded error, given only a uniform approximation.  In Section~\ref{sec:poa}, we give an example of a property---the price of anarchy---for which \naive{} estimation via a uniform approximation %
can be arbitrarily incorrect.


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}



\begin{remark}[Estimation Complexity]
While estimating an arbitrary game requires estimating $\NumberOfPlayers\prod_{i=1}^{\NumberOfPlayers}|\StrategySet_\PlayerIndex|$ parameters, many games of practical importance require far fewer parameters. For example, in symmetric games, where all players have the same strategy set $\StrategySet$, there are only ${\NumberOfPlayers + |\StrategySet| - 1 \choose \NumberOfPlayers}$ many pure strategy profiles . 

\end{remark}


\begin{remark}[Limitations of Uniform Approximations]
Some properties of games are unstable under $\epsilon$-perturbations (e.g., even $\epsilon$-uniform approximations).
For example, whether a strategy is $\gamma$-rationalizable may depend on whether another strategy is $\epsilon$-rationalizable (due to IEDS), and the gap between $\gamma$ and $\epsilon$ may be arbitrarily wide.
\textbf{For instance, whether a strategy is rationalizable depends on which other strategies are rationalizable; thus, if it is ambiguous whether strategy $\Strategy_1$ of agent 1 is dominated by strategy $\Strategy_2$, it can be ambiguous whether strategy $\Strategy_3$ of agent 2 is rationalizable, as it could be dominated (by an arbitrarily large margin) by strategy $\Strategy_4$ of agent 2, \emph{unless\/} agent 1 plays $\Strategy_1$.}
Consequently, while estimating $\epsilon$-minimax strategies is possible, estimating $\epsilon$-minimax strategies under the common knowledge of rationality assumption (i.e., no dominated strategies) is not.
\end{remark}


==> finite-congestion-games.tex <==
\section{Finite Congestion Model}
A {\it finite congestion game}~\cite{christodoulou2005price} is a tuple $\CongestionGame = (\SetOfPlayers, \SetOfFacilities, (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}, (\FacilityCostFunction)_{\FacilityIndex\in\SetOfFacilities})$,
where $\SetOfPlayers = \{1, \ldots, \NumberOfPlayers\}$ is a set of players, $\SetOfFacilities = \{1, \ldots, \NumberOfFacilities\}$ is a set of facilities,
$(\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers} \subseteq 2^\NumberOfFacilities$ is the set of pure strategies for player $\PlayerIndex$. A strategy $\Strategy_\PlayerIndex \in \SetOfStrategies_\PlayerIndex$ is a set of facilities. Finally, $\FacilityCostFunction_\FacilityIndex$ is a cost function associated with facility $\FacilityIndex$.

A pure strategy profile $\Strategy = (\Strategy_1, \ldots, \Strategy_\NumberOfPlayers)$ is a vector of strategies, one for each player. In a finite congestion game, each player selects a strategy so as to minimize their costs. Given a profile of strategies $\Strategy$, the cost for player $\PlayerIndex$ for $\Strategy$ is defines as $\PlayerCost_\PlayerIndex(\Strategy) = \sum_{\FacilityIndex\in\Strategy_\PlayerIndex} \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex(\Strategy))$, where $\NumberOfPlayers_\FacilityIndex(\Strategy)$ is the number of players selecting facility $\FacilityIndex$ in $\Strategy$.

A {\it pure strategy profile} is a Nash equilibrium if no player has an incentive to unilaterally deviate to another pure strategy. Mathematically, $\Strategy^*$ is a pure Nash equilibirum if $\forall \PlayerIndex \in \SetOfPlayers, \forall \Strategy_\PlayerIndex \in \SetOfStrategies_\PlayerIndex: \PlayerCost_\PlayerIndex(\Strategy^*) \le \PlayerCost_\PlayerIndex(\Strategy^*_{-\PlayerIndex}, \Strategy_\PlayerIndex)$, where $(\Strategy^*_{-\PlayerIndex}, \Strategy_\PlayerIndex)$ is the strategy profile obtained if just player $\PlayerIndex$ deviates from $\Strategy^*_\PlayerIndex$ in $\Strategy^*$. 
In~\cite{rosenthal1973class} it was shown that this class of games have at least one pure Nash equilibria provided that each facility's cost function $\FacilityCostFunction_\FacilityIndex$ is a function of the number of players selecting that facility only, i.e., $\FacilityCostFunction_\FacilityIndex = \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex)$.

The {\it system's cost} of strategy $\Strategy$ is defined as the sum of the cost incurred by each player in $\Strategy$ which we denote by $\SystemCost(\Strategy) = \sum_{\PlayerIndex\in\SetOfPlayers} \PlayerCost_\PlayerIndex(\Strategy)$. The optimal system's cost is defined as $\SystemCost^* = \min\limits_{\Strategy \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}} \SystemCost(\Strategy)$
\section{Price of Anarchy}
The ratio between the worst possible system's cost of a Nash equilibrium (in mixed or pure strategies) and the optimum system's cost was first proposed in \cite{koutsoupias1999worst} as a measure of the effectiveness of a system and later dubbed the {\it price of anarchy}~\cite{papadimitriou2001algorithms,roughgarden2002bad}. Since congestion games always have a pure Nash equilibrium, is natural to investigate the {\it pure price of anarchy} (PPA) where one considers only Nash equilibria in pure strategy in this class of games. Mathematically, the PPA of a finite congestion game $\PurePriceOfAnarchy(\CongestionGame)$ is defined as follows.
\begin{definition}[The pure price of anarchy (PPA)]
Let $\CongestionGame$ be a congestion game (in general, any game for which pure Nash equilibria is guaranteed to exists). 
We denote the pure price of anarchy (PPA) of $\CongestionGame$ by $\PurePriceOfAnarchy(\CongestionGame)$ and define it as:
\begin{equation}
    \PurePriceOfAnarchy(\CongestionGame) = \dfrac{\max\limits_{\{\Strategy^* \in (\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}
                                                \mid \Strategy^* \text{ is a pure Nash equilibrium}\}} \SystemCost(\Strategy^*)}
                                             {\SystemCost^*}
\label{eq:PPA}
\end{equation}
\label{def:PPA}
\end{definition}
Most known theoretical results for pure price of anarchy in finite congestion games make strong assumptions about the functional form of $\FacilityCostFunction_\FacilityIndex$. For example, authors in~\cite{christodoulou2005price} showed that when $\FacilityCostFunction_\FacilityIndex(k) = k$, the PPA is 5/2.
\begin{example}
Consider the following example of a finite congestion game due to~\cite{christodoulou2005price}. There are 3 players and 6 facilities. Partition the set of facilities in two, $\SetOfFacilities_1 = \{h_1, h_2, h_3\}$ and $\SetOfFacilities_2 = \{g_1, g_2, g_3\}$. Each player has two strategies: $\SetOfStrategies_1 = \{\{h_1, g_1\}, \{g_2, h_3, h_2\}\}, $
$\SetOfStrategies_2 = \{\{h_2, g_2\}, \{g_2, h_3, h_2\}\},$ and
$\SetOfStrategies_1 = \{\{h_3, g_3\}, \{g_1, h_2, h_1\}\}$. If the cost of facilities is given by $\FacilityCostFunction_\FacilityIndex(k) = k$ for all $\FacilityIndex \in \SetOfFacilities_1 \cup \SetOfFacilities_2$, then one can verify that the profiles of strategies $\Strategy_1 = (\{h_1, g_1\}, \{h_2, g_2\}, \{h_3, g_3\})$ and $\Strategy_2 = (\{g_2, h_3, h_2\}, \{g_2, h_3, h_2\}, \{g_1, h_2, h_1\})$ are both Nash equilibria. In this case, $\Strategy_1$ is the social optimum with $\SystemCost(\Strategy_1) = 3 \cdot 2$ while $\SystemCost(\Strategy_2)=3 \cdot 5$. Note that this implies a PPA of 5/2.
\label{ex:PPA}
\end{example}
\subsection{The $\epsilon$-Pure Price of Anarchy}
Since we are interested in solving games that are too complex to be amenable to analytical solutions, we define a notion of $\epsilon$-price of anarchy which is amenable to estimation from data. 
\begin{definition}[The $\epsilon$-pure price of anarchy ($\epsilon$-PPA)]
Let $\epsilon > 0$ and $\CongestionGame$ be a congestion game (in general, any game). 
We define the $\epsilon$-pure price of anarchy as the following ratio
\begin{equation}
    \PurePriceOfAnarchy_\epsilon(\CongestionGame) = 
    \dfrac
{\max\limits_{\{\mathbb{\Strategy^*} \mid \mathbb{\Strategy^*} \text{is an $\epsilon$-sink equilibrium}\}} \SystemCost(\mathbb{\Strategy^*})}
{\min\limits_{\{\mathbb{\Strategy^*} \mid \mathbb{\Strategy^*} \text{is an $\epsilon$-sink equilibrium of the UM graph}\}} \SystemCost(\mathbb{\Strategy^*})}
\label{eq:epsPPA}
\end{equation}
\label{def:epsPPA}
\end{definition}
Note that we overload notation and used $\SystemCost(\mathbb{\Strategy})$ to denote the cost of sink $\mathbb{\Strategy} = \{\Strategy_1, \ldots, \Strategy_k\}$. We still need to define exactly which metric we care about for a sink, e.g., average cost would be $\SystemCost(\mathbb{\Strategy}) = \SystemCost(\{\Strategy_1, \ldots, \Strategy_k\}) = \dfrac{1}{k}\sum_{l=1}^k \SystemCost(\Strategy_l)$. (Note to self, for $\epsilon$ large enough, $\PurePriceOfAnarchy_\epsilon$ is always 1).

A few more comments about Definition~\ref{def:epsPPA}. Note that in the numerator we consider the worst possible {\it $\epsilon$-sink equilibrium} instead of the worst possible $\epsilon$-pure Nash as we did for Definition~\ref{def:PPA} (formal definition of $\epsilon$-sink equilibria pending but in a nutshell: a sink of the $\epsilon$-best response graph is an $\epsilon$-sink equilibrium). 
The reason is simple: once we relax the Nash solution concept to $\epsilon$-Nash, 

we no longer have a guarantee of existence in pure strategies, even for congestion games. Consequently, we instead consider sink equilibria, which is the natural generalization of pure Nash equilibria, but of course, up to an $\epsilon$ error. 

Using our current tools, we can estimate both numerator and denominator. Note, however, that we can estimate the numerator with probability at least $1 - \delta_n$ and denominator with probability $1 - \delta_d$. Consequently, we can estimate the ratio with probability $(1-\delta_n)(1-\delta_d)$.


\section{Mechanism Design}
Suppose now we take the role of a {\it mechanism designer} trying to modify the rules of a finite congestion game so as to minimize the overall congestion across all players. Suppose we have access to players' preferences (understood here as the set of strategies $(\SetOfStrategies_\PlayerIndex)_{\PlayerIndex\in\SetOfPlayers}$) but we are not allowed to change them as these are set by the players a priori. Instead, as the designers, we can only change the cost functions for different facilities. In this case, we next illustrate, in the context of example~\ref{ex:PPA}, how one can chose cost functions so as to minimize the price of anarchy.

{\it {\bf Remark}: Note that as currently formulated, we don't believe this example makes a lot of sense. The problem that we have is that the denominator in the calculation of PPA -equation~(\ref{eq:PPA})- is not fixed but may vary as a function of the cost of the facilities. In particular, note how in the new game we have a higher cost in the optimal system's cost than in the optimal system's cost of the original game but still a lower system's cost than in the bad Nash of the original game. This means that we have sacrificed a potential lower overall cost for a higher cost that is more likely to be played. In other words, we have reduced the price of anarchy but in the process we have change the value of the optimal solution, something we believe to be an undesirable property.}
\begin{example} 
Let us consider the following variation of example~\ref{ex:PPA}. If we define  $\FacilityCostFunction_g(k) = k$ for $g \in \SetOfFacilities_1$ and
$\FacilityCostFunction_h(k) = 2k$ for $h \in \SetOfFacilities_2$, then in the ensuing game strategy $\Strategy_1$ will be the unique pure Nash equilibrium. Moreover, the unique pure Nash will coincide with the optimal system's cost, i.e., the strategy profile with minimum overall cost. Note that in this case the PPA is 1.

This example illustrates the possibility of using mechanism design to select the parameters of the game (in the above example, the facilities' cost functions where we restrict to select only their slope) to optimize a designers' objective function (in the example, the PPA). \end{example}
\section{Experiments}
In this section, we investigate the empirical performance of our algorithms. 
\subsection{Experimental Setup}
We experiment with a distribution of random, finite congestion games which we call $RFC(\NumberOfPlayers, \NumberOfFacilities)$ consisting of games $\CongestionGame$ with $\NumberOfPlayers$ players and $\NumberOfFacilities$ facilities. The cost for player $i$ is defined as 
$\PlayerCost_\PlayerIndex(\Strategy) = \sum_{\FacilityIndex\in\Strategy_\PlayerIndex} \FacilityCostFunction_\FacilityIndex(\NumberOfPlayers_\FacilityIndex(\Strategy)) + \xi$ where $\xi$ is a random noise.


What remains to model are (1) the topology of preferred strategies for each player (these should model some interesting situation), and (2) the form of the facilities' costs and the form of the noise (note that we know that only for simple form of facilities' costs we have bounds on the PPA). 

The following are proposals for both (1) and (2).

\subsubsection{Players' preferences}
I propose we test the following topologies for players' preferences. 

\underline{Power Law}: under this topology, each player $\PlayerIndex$ has a random number of pure strategies $n_\PlayerIndex \sim U[a, b]$ where $a < b \in \{1,\ldots, 10\}$. Note that $n_\PlayerIndex \le 2^{\NumberOfFacilities}-1$. Each pure strategy  $\Strategy_{\PlayerIndex, k}$, where $k \in \{1, \ldots, n_\PlayerIndex\}$ is constructed as follow. The probability that facility $j \in \{1, \ldots, \NumberOfFacilities\}$ is in $\Strategy_{\PlayerIndex, k}$ is given by a simple power law $p[j \in \Strategy_\PlayerIndex] = \alpha^{-j}$, where $\alpha \in [0,1]$ is a free parameter. Note that we have the option of enforcing a hard requirement of $n_\PlayerIndex$ strategies, or we may allow strategy repetitions in which case $n_\PlayerIndex$ is just an upper bound on the number of strategies for player $\PlayerIndex$. 

The interpretation of $\alpha$ is that for higher (lower) values of $\alpha$ we model a system with a more (less) diverse set of preferred facilities. In this model, we chose facilities independent of each other. This model then correspond to a situation where there is a clearly preferred facility, e.g., a very busy metro station, and other less preferred facilities, e.g., stations at the outskirts of a city. 

However, a more interesting/complex model would be one where the probability of selecting a facility is influenced by the probabilities of other facilities (for example, to go back home from work in the metro, one may need to change stations and thus, stations that are close to each other in certain paths are preferable). In this case, one could have an underlying graph (e.g., map of Tokyo metro) of preferences (can we use CATS for this?). 

\subsubsection{Noise}
We could start with simple Gaussian noise $\xi \sim \mathcal{N}(\mu, \sigma)$ for suitable choices of $\mu, \sigma$, and/or uniform noise $\xi \sim U(c, d)$ for suitable choices of $c < d$. However, since congestion games as described in this document are finite and discrete, I find it hard to interpret continuous noise in this model. An alternative is to introduce discrete noise, for example, by using a geometric distribution. This last noise model the situation where we can't measure exactly the number of people selecting a facility but instead can only have an integer approximation.
\subsection{Metrics}
We need metrics for at least:
\begin{enumerate}
    \item Sample complexity (e.g., how many samples as a function of $\epsilon,\delta$)
    \item System's cost (and maybe individuals' costs)
    \item Accuracy of outcomes, if ground-truth is known (e.g., for instances where we know (or have bounds on) the PPA). How long and how many samples does it take to get the right answer?
    \item Time complexity.
    \item Proportion of outcomes where the algorithm fails (an empirical measure of $\delta$).
\end{enumerate}


==> noise_scaling.tex <==




\begin{theorem}[Noise Scaling]
\label{thm:ra-vns}

Suppose conditional normal-form game $\ConditionalGame{\ConditionSpace}$, distribution $\ConditionDistribution$, and index set $\Indices$, such that for all $(\PlayerIndex, \StratProfile) \in \Indices$,
\[
\hat{\Utility}_\PlayerIndex(\StratProfile; \Samples) = \Utility_{\PlayerIndex}(\StratProfile; \ConditionDistribution) + \eta_{\PlayerIndex}(\StratProfile; \Samples) \enspace,
\]
\todo{Better explanation of what $F$ is.}
where $\eta_\PlayerIndex(\StratProfile; \Samples)$ is an arbitrary real-valued function.  Furthermore, take
\[
F(v) \doteq \abs{\left\{ (\PlayerIndex, \StratProfile) \in \Indices \ \middle| \ \sup_{\Samples \in \ConditionSpace} \abs{\eta_\PlayerIndex(\StratProfile; \Samples)} \leq v \right\}} \text{and} \enspace F(v_1, v_2) \doteq F(v_2) - F(v_1) \enspace,
\]
and suppose $\sup_{(\PlayerIndex, \StratProfile) \in \Indices} \abs{\Utility_{\PlayerIndex}(\StratProfile; \ConditionDistribution)} \leq a$.  Then, for any sequence $v_0, v_1, v_2, \dots, v_n$ such that $v_0 = 0$ and $v_n = c$, we may bound the Rademacher average as
\[
\RC{\NumberOfSamples}{\GameTuple, \Indices}{\ConditionDistribution} \leq \frac{a}{\sqrt{\NumberOfSamples}} + \sum_{i=1}^n v_i\min\left(1, \sqrt{\frac{\ln(F(v_{i-1}, v_{i}))}{2\NumberOfSamples}}\right) \enspace.
\]
\end{theorem}
\begin{proof}
This proof is structurally quite similar to the proof of \Cref{thm:ra-factored}.  The expected utilities are extracted and handled through the same random-walk / binomial mean absolute deviation argument (marked \textsc{See Above} in the proof), though now instead of the triangle inequality, a nonnegative suprema-summation inequality is now used to split the Rademacher average (a similar strategy is used to prove Theorem~3.3 of \citep{boucheron2005theory}).

First take $\Indices_i \doteq \{ (\PlayerIndex, \StratProfile) \in \Indices \ | \ v_{i-1} < \abs{\sup_{x \in \ConditionSpace} \Utility_{\PlayerIndex}(\StratProfile; \ConditionDistribution)} \leq v_i\}$, and note that $\abs{\Indices_i} = F(v_i) - F(v_{i-1})$.  Technically, this construction can result in suprema over empty sets and logarithms of $0$, which in both cases must be resolved as 0 (intuitively, we can add the $0$ function to any function family without increasing the Rademacher average, and the Rademacher average of the function family containing only the $0$ function is $0$).

\begin{align*}
\RC{\NumberOfSamples}{\GameTuple, \Indices}{\ConditionDistribution} \hspace{-1cm} & \hspace{1cm} = \Expwrt{\vsigma,\Samples}{\sup_{(\PlayerIndex, \StratProfile) \in \Indices} \abs{\frac{1}{\NumberOfSamples} \sum_{\SampleIndex=1}^{\NumberOfSamples} \vsigma_\SampleIndex \Utility_\PlayerIndex(\StratProfile; \SamplePoint_\SampleIndex)} } & \textsc{Definition of $\RC{\NumberOfSamples}{\GameTuple, \Indices}{\ConditionDistribution}$} \\
 &\leq \frac{a}{\sqrt{\NumberOfSamples}} + \Expwrt{\vsigma,\Samples}{\sup_{(\PlayerIndex, \StratProfile) \in \Indices_i} \abs{ \sum_{i=1}^{n} \frac{1}{\NumberOfSamples} \sum_{\SampleIndex=1}^{\NumberOfSamples} \vsigma_\SampleIndex \eta_\PlayerIndex(\StratProfile; \SamplePoint_\SampleIndex)}} & \textsc{See Above} \\
 &\leq \frac{a}{\sqrt{\NumberOfSamples}} + \sum_{i=1}^{n}\Expwrt{\vsigma,\Samples}{\sup_{(\PlayerIndex, \StratProfile) \in \Indices_i} \abs{\frac{1}{\NumberOfSamples} \sum_{\SampleIndex=1}^{\NumberOfSamples} \vsigma_\SampleIndex \eta_\PlayerIndex(\StratProfile; \SamplePoint_\SampleIndex)}} & \begin{tabular}{r} $\displaystyle\sup_{\mathclap{a \in \bm{A} \cup \bm{A}'}} \abs{a} \leq \sup_{a \in \bm{A}} \abs{a} + \sup_{\mathclap{a' \in \bm{A}'}} \abs{a'}$ \\ \textsc{Linearity of Expectation} \end{tabular} \hspace{-0.19cm} \\
 &\leq \frac{a}{\sqrt{\NumberOfSamples}} + \sum_{i=1}^n v_i \min\left(1, \sqrt{\frac{\ln(F(v_{i-1}, v_{i}))}{2\NumberOfSamples}}\right) & \textsc{Massart's Inequality}
\end{align*}


\end{proof}



\iftrue %
\begin{figure}

\begin{multicols}{2}

\begin{tikzpicture}

\begin{axis}[
        no markers,
        domain=1:100,
        samples=35,smooth,
        legend pos=north west,
        legend style={draw=none,fill=none,font=\scriptsize},
        width=3.5in,
        height=2in,
        xticklabel style={
            font=\small
        },
        yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=3,
            font=\small
        },
        scaled y ticks=false,
        xlabel={Number of Agents $\NumberOfPlayers$},
        label style={font=\small},
        xmin=0,xmax=100,
    ]

\addplot[style=solid,color=blue]{2 * sqrt((ln(2) + ln(x) + x * ln(\na) - ln(\del)) / (2 * \ns))};
\addlegendentry{Hoeffding: $\norm{\bm{a}}_{\!1}\mathsmaller{\sqrt{\nicefrac{2\ln({2\NumberOfPlayers\NumberOfStrategies^{\NumberOfPlayers}}{\delta})}{m}}}\hspace{0.5cm}$};

\addplot[style=solid,color=red]{2 * (1 / sqrt(\ns) + (1 / 32) * sqrt((ln(2 * x / 2) + x * ln(\na)) / (2 * \ns)) + 0.25 * sqrt((ln(2 * x / 4) + x * ln(\na)) / (2 * \ns)) + 0.125 * sqrt((ln(2 * x / 8) + x * ln(\na)) / (2 * \ns)) + 0.25 * sqrt((ln(2 * x) - ln(16) + x * ln(\na)) / (2 * \ns)) + 0.5 * sqrt((ln(2 * x) - ln(32) + x * ln(\na)) / (2 * \ns)) + 1 * sqrt((ln(2 * x) - ln(64) + x * ln(\na)) / (2 * \ns))) + 2 * 3 * sqrt(-ln(\del) / (2 * \ns))};
\addlegendentry{Rademacher: $\leq 2\RC{m}{\GameTuple, \SetOfPlayers \times \StratProfileSpace}{\rand{D}} + 3\norm{\bm{a}}_{\!1}\mathsmaller{\sqrt{\nicefrac{2\ln(1/\delta)}{m}}}$};

\end{axis}
\end{tikzpicture}

\vfill\columnbreak

\if 0
\[
F(v) \leq \floor{v^{-p}}\abs{\NumberOfPlayers}
\]

\[
v_i = \frac{i}{n}
\]
\fi

\[
F(v_{i-1}, v_{i}) \leq \ceil{\frac{\NumberOfPlayers\NumberOfStrategies^{\NumberOfPlayers}}{2^{i}}}
\]

\[
a = 1, c = 2
\]

\end{multicols}
\caption{Rademacher vs.\ Hoeffding Bounds for Variable-Scale Noise Game with (variable) $\NumberOfPlayers$, $\NumberOfStrategies$, $\NumberOfSamples = 100$ samples, and $\delta = 0.05$.}
\label{fig:variable-noise-scale-games}
\end{figure}
\fi


